VecGAN: Image-to-Image Translation with Interpretable Latent Directions

We propose VecGAN, an image-to-image translation framework for facial attribute editing with interpretable latent directions. Facial attribute editing task faces the challenges of precise attribute editing with controllable strength and preservation of the other attributes of an image. For this goal, we design the attribute editing by latent space factorization and for each attribute, we learn a linear direction that is orthogonal to the others. The other component is the controllable strength of the change, a scalar value. In our framework, this scalar can be either sampled or encoded from a reference image by projection. Our work is inspired by the latent space factorization works of fixed pretrained GANs. However, while those models cannot be trained end-to-end and struggle to edit encoded images precisely, VecGAN is end-to-end trained for image translation task and successful at editing an attribute while preserving the others. Our extensive experiments show that VecGAN achieves significant improvements over state-of-the-arts for both local and global edits.

==> additional_exp.tex <==

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Configuration}}} & \multicolumn{2}{c}{\textbf{Realism FID}}                                                                  & \multicolumn{2}{c|}{\textbf{Disentanglement FID}}                                                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                        & \multicolumn{1}{c}{\textbf{Latent-guided}} & \multicolumn{1}{c|}{\textbf{Reference Guided}} & \multicolumn{1}{c}{\textbf{Latent-guided}} & \multicolumn{1}{c|}{\textbf{Reference Guided}} \\ \hline
SDIT \cite{wang2019sdit} & 33.73 & 33.12 & 80.25 & 79.72\\
StarGANv2 \cite{starganv2} & 26.04 & 25.49 & 90.08 & 78.03\\
HiSD \cite{li2021image} &  21.37 &  21.49 &  71.85 & 71.48 \\

HiSD 128x128(trained)  &  21.35 & 22.55 & 71.69 & 72.94 \\
v1 - Single Discriminator & 26.27 & 26.84 & 78.15 & 78.36 \\
v2 - Double Discriminator & 27.18 & 26.38 & 79.45 & 77.77 \\
v3 - Self translation (170k) & 26.49 & 26.33 & 77.70 & 77.93 \\
v4 - Deeper encoder/decoder (120k) & 24.08 & 24.19 & 74.71 & 75.03\\
v4 - Deeper encoder/decoder (150k) & 23.69 & 23.76 & 75.23 & 74.74 \\
v4 - Deeper encoder/decoder (190k) & 23.70 & 23.53 & 74.09 & 74.15 \\
v4 - Deeper encoder/decoder (200k) & 26.27 & 26.49 & 76.16 & 76.74 \\
v5 - Skip connections (70k) & 23.93 & 23.59 & 74.70 & 74.27 \\
v5 - Skip Connections (160k) & 25.52 & 24.99 & 76.52 & 76.03 \\
v6 - Shift discriminator (160k) & 24.97 & 25.15 & 77.64 & 77.87 \\
v6 - Shift discriminator (200k) & 25.07 & 23.71 & 77.34 & 75.30 \\
v7 - no skip connections - 8x8 & 37.31 & 29.55 & 86.13 & 78.03 \\
v8 (128-8x8) - Attention skip (110k) & 24.11 & 23.39 & 75.42 & 73.69 \\
v8 (256-8x8) - Attention skip (100k) & 23.15 & 23.17 & 74.29 & 74.03 \\
v9 - Learnable orthagonality (200k) & 23.25 & 23.50 & 73.66 & 73.66 \\
v9 - Shift discriminator (alpha + tag) (270k) & 21.75 & 21.74 & 73.16 & 73.06 \\

\hline
\end{tabular}}
    \caption{Evaluation results for experiments}
    \label{tab:HiSD results}
\end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Iteration}}} & \multicolumn{2}{c}{\textbf{Realism FID}}                                                                  & \multicolumn{2}{c|}{\textbf{Disentanglement FID}}                                                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                        & \multicolumn{1}{c}{\textbf{Latent-guided}} & \multicolumn{1}{c|}{\textbf{Reference Guided}} & \multicolumn{1}{c}{\textbf{Latent-guided}} & \multicolumn{1}{c|}{\textbf{Reference Guided}} \\ \hline
90k & 24.18 & 23.03 & 75.67 & 73.82 \\
100k & 23.07 & 23.12 & 74.36 & 73.76 \\
110k & 23.47 & 23.48 & 74.68 & 74.59 \\
120k & 24.69 & 24.57 & 76.22 & \\
200k & 24.46 & 24.14 & 75.34 & 75.21\\
\end{tabular}}
    \caption{Evaluation over iterations for the optimum model (256-8x8) - Attention skip (100k)}
    \label{tab:over_iters}
\end{table*}




\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Configuration}}} & \multicolumn{2}{c}{\textbf{Realism}}                                                                  & \multicolumn{2}{c|}{\textbf{Disentanglement}}                                                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                        & \multicolumn{1}{c}{\textbf{L}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c}{\textbf{L}} & \multicolumn{1}{c|}{\textbf{R}} \\ \hline
HiSD \cite{li2021image} &  21.37 &  21.49 &  71.85 & 71.48 \\
HiSD (32x32)  &  21.35 & 22.55 & 71.69 & 72.94 \\
HiSD (16x16)   \\
HiSD (8x8)  \\
HiSD (4x4)  \\
\hline
\end{tabular}
    \caption{Evaluation results for experiments}
    \label{tab:HiSD_abl}
\end{table}


\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Configuration}}} & \multicolumn{2}{c}{\textbf{Realism}}                                                                  & \multicolumn{2}{c|}{\textbf{Disentanglement}}                                                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                        & \multicolumn{1}{c}{\textbf{L}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c}{\textbf{L}} & \multicolumn{1}{c|}{\textbf{R}} \\ \hline

Ours (32x32)  & 26.27 & 26.84 & 78.15 & 78.36  \\
Ours (16x16) & 23.70 & 23.53 & 74.09 & 74.15   \\
Ours (8x8)  \\
Ours (4x4)  \\
\hline
\end{tabular}
    \caption{Evaluation results for experiments}
    \label{tab:ours_abl}
\end{table}
